Differentially Private Gomory-Hu Trees

Given an undirected, weighted $n$-vertex graph $G = (V, E, w)$, a Gomory-Hu tree $T$ is a weighted tree on $V$ that preserves the Min-$s$-$t$-Cut between any pair of vertices $s, t \in V$. Finding cuts in graphs is a key primitive in problems such as bipartite matching, spectral and correlation clustering, and community detection. We design a differentially private (DP) algorithm that computes an approximate Gomory-Hu tree. Our algorithm is $\varepsilon$-DP, runs in polynomial time, and can be used to compute $s$-$t$ cuts that are $\tilde{O}(n/\varepsilon)$-additive approximations of the Min-$s$-$t$-Cuts in $G$ for all distinct $s, t \in V$ with high probability. Our error bound is essentially optimal, since [Dalirrooyfard, Mitrovi\'c and Nevmyvaka, NeurIPS 2023] showed that privately outputting a single Min-$s$-$t$-Cut requires $\Omega(n)$ additive error even with $(\varepsilon, \delta)$-DP and allowing for multiplicative error. Prior to our work, the best additive error bounds for approximate all-pairs Min-$s$-$t$-Cuts were $O(n^{3/2}/\varepsilon)$ for $\varepsilon$-DP [Gupta, Roth and Ullman, TCC 2012] and $\tilde{O}(\sqrt{mn}/ \varepsilon)$ for $(\varepsilon, \delta)$-DP [Liu, Upadhyay and Zou, SODA 2024], both achieved by DP algorithms that preserve all cuts in the graph. To achieve our result, we develop an $\varepsilon$-DP algorithm for the Minimum Isolating Cuts problem with near-linear error, and introduce a novel privacy composition technique combining elements of both parallel and basic composition to handle `bounded overlap' computational branches in recursive algorithms, which may be of independent interest.

==> updated_stcut.tex <==
\begin{proofof}{Claim \ref{claim:stcut}}
\mina{copied most of it from our paper}
    Let $G$ and $G'$ be two neighboring graphs.
    Let edge $e = uv$ be the one for which $w_e$ in $G$ and $G'$ differ; recall that it differs by at most $\tau$. To analyze the probability with which Algorithm outputs the same cut for input $G$ as it outputs for input $G'$, we first sample all the $X_{z, x}$ for $x \in V \setminus \{u, v\}$.
    Intuitively, the outcomes of those random variables are not crucial for the difference between outputs of Algorithm invoked on $G$ and $G'$. We now elaborate on that.

    Consider \textbf{all} the $s$-$t$ cuts -- not only the minimum ones -- in $G$ before $X_{z, u}$ and $X_{z, v}$ are sampled; for instance, assume for a moment that those two random variables equal $0$. 
    Let $\allcuts(G)$ be all those cuts sorted in a non-decreasing order with respect to their weight.
    Observe that $\allcuts(G) = 2^{n - 2}$. As we will show next, although there are exponentially many cuts, we will point to only four of them as crucial for our analysis. This will come in very handy in the rest of this proof.
    We now partition $\allcuts(G)$ into four groups based on which $u$ and $v$ are on the same side of the cut as $z$. Let $\cC_u(G)$ be the subset of $\allcuts(G)$ for which $u$ is on the same side of a cut as $z$ while $v$ is on the other side. Analogously we define $\cC_v(G)$. We use $\cC_{u, v}(G)$ to represent the subset of $\allcuts(G)$ for which $z$, $u$, and $v$ are all on the same side. Finally, by $\cC_{\emptyset}(G)$ we refer to the subset of $\allcuts(G)$ for which $u$, and $v$ are all on the side that doesn't contain $z$.

    Let $C_u$, $C_v$, $C_{u,v}$, and $C_\emptyset$ be the min cuts in $\cC_u(G)$, $\cC_v(G)$, $\cC_{u, v}(G)$, and $\cC_\emptyset(G)$, respectively, before $X_{z, u}$ and $X_{z, v}$ are sampled.
    It is an easy observation that sampling $X_{z, u}$ and $X_{z, v}$ and altering the weight of the edge $e$ changes the weight of all the cuts in $\cC_u(G)$ by the same amount. This same observation also holds for $\cC_v(G)$, $\cC_{u, v}(G)$ and $\cC_{\emptyset}(G)$. 
    This further implies that the min $s$-$t$ cut of $G$ after $X_{z, u}$ and $X_{z, v}$ are sampled will be among $C_u$, $C_v$, $C_{u,v}$, and $C_\emptyset$.
    Observe that these four cuts are also the minimum-weight cuts in $\cC_u(G')$, $\cC_v(G')$, $\cC_{u, v}(G')$, and $\cC_{\emptyset}(G')$, respectively.

    In other words, the min $s$-$t$ cuts in $G$ and in $G'$ are among $C_u$, $C_v$, $C_{u,v}$ and $C_\emptyset$, but not necessarily the same; this holds both before and after sampling $X_{z, u}$ and $X_{z, v}$. In the rest of this proof, we show that sampling $X_{z, u}$ and $X_{z, v}$ makes it likely that the min $s$-$t$ cuts in $G$ and $G'$ are the same cut.


    \paragraph{The ratio of probabilities in $G'$ and $G$ that $C_u$ is the min $s$-$t$ cut.}
    Simply, our goal is to compute
    \begin{equation}
        \frac
        {\prob{w_{G'}(C_u) < w_{G'}(C_v)\ \wedge\ w_{G'}(C_u) < w_{G'}(C_{u,v})\ \wedge\ w_{G'}(C_u) < w_{G'}(C_{\emptyset})}}
        {\prob{w_G(C_u) < w_G(C_v)\ \wedge\ w_G(C_u) < w_G(C_{u,v})\ \wedge\ w_G(C_u) < w_G(C_{\emptyset})}}. \label{eq:huge-ratio}
    \end{equation}

    First consider the case $w_{G}(e) = w_{G'}(e) + \tau$, for some $\tau > 0$. 
    For the ease of calculation, for $x \in \{\emptyset, \{u, v\}\}$, define $\Delta_x = w_G(C_u) - w_G(C_x)  - \tau$ and define $\Delta_v = w_G(C_u) - w_G(C_v)$ \emph{before} $X_{z, u}$ and $X_{z, v}$ are sampled. In the rest of this proof, we are analyzing the behavior of cuts when $X_{z, u}$ and $X_{z, v}$ {\bf are sampled}.
    Then, we have
    \begin{align}
          & \prob{w_G(C_u) < w_G(C_v)\ \wedge\ w_G(C_u) < w_G(C_{u,v})\ \wedge\ w_G(C_u) < w_G(C_{\emptyset})} \nonumber \\
        = & \Pr[\Delta_v + X_{z,v} < X_{z, u} \wedge\ \Delta_{u, v} + X_{z, v} + \tau < 0\ \wedge\ \Delta_{\emptyset} + \tau <  X_{z, u}]\nonumber \\
        = & \prob{X_{z,v} - X_{z,u} < -\Delta_v\ \wedge\ X_{z,v} < -\Delta_{u, v} - \tau \ \wedge\ -X_{z,u} < -\Delta_\emptyset - \tau}
        \label{eq:w_H(C_u)-upper-bound}
    \end{align}
    Now, we replace $X_{z,v}$ by $x$ and $-X_{z,u}$ by $y$.
    Then, \cref{eq:w_H(C_u)-upper-bound} can be rewritten as
    \begin{align*}
        & \prob{w_G(C_u) < w_G(C_v)\ \wedge\ w_G(C_u) < w_G(C_{u,v})\ \wedge\ w_G(C_u) < w_G(C_{\emptyset})} \\
        = & \prob{x + y < -\Delta_v\ \wedge\ x < -\Delta_{u, v} - \tau \ \wedge\ y < -\Delta_\emptyset - \tau}.
    \end{align*}
    Applying the same analysis for $G'$ we derive
    \begin{align*}
    & \prob{w_{G’}(C_u) < w_{G’}(C_v)\ \wedge\ w_{G’}(C_u) < w_{G’}(C_{u,v})\ \wedge\ w_{G’}(C_u) < w_{G’}(C_{\emptyset})} \nonumber \\
    = & \Pr[\Delta_v + X_{z,v} <  X_{z, u} \ \wedge\ \Delta_{u, v} + X_{z, v} < 0\ \wedge\ \Delta_{\emptyset}  < X_{z, u}].
    \end{align*}
    Replacing $X_{z,v}$ by $x$ and $-X_{z,u}$ by $y$ yields
    \begin{align*}
        & \prob{w_{G'}(C_u) < w_{G'}(C_v)\ \wedge\ w_{G'}(C_u) < w_{G'}(C_{u,v})\ \wedge\ w_{G'}(C_u) < w_{G'}(C_{\emptyset})} \\
        = & \prob{x + y < -\Delta_v\ \wedge\ x < -\Delta_{u, v} \ \wedge\ y < -\Delta_\emptyset}.
    \end{align*}
    Note that we have that $x$ and $y$ follow $\Lap(1/\eps)$. Moreover, observe that the random variables $x$ and $y$ are independent by definition. Therefore, by invoking \cref{lemma:a-mish-mash-of-two-Lap-rv} with $\alpha = -\Delta_{u,v} - \tau$, $\beta = -\Delta_\emptyset - \tau$, and $\gamma = -\Delta_v$ we derive
    \[
        \frac
        {\prob{w_{G'}(C_u) < w_{G'}(C_v)\ \wedge\ w_{G'}(C_u) < w_{G'}(C_{u,v})\ \wedge\ w_{G'}(C_u) < w_{G'}(C_{\emptyset})}}
        {\prob{w_G(C_u) < w_G(C_v)\ \wedge\ w_G(C_u) < w_G(C_{u,v})\ \wedge\ w_G(C_u) < w_G(C_{\emptyset})}} \le e^{4 \tau \eps}.
    \]


    Considering the second case $w_{G}(e) + \tau = w_{G'}(e)$, for some $\tau > 0$, we derive that the ratio \cref{eq:huge-ratio} is upper-bounded by $1 \le e^{4 \tau \eps}$.


    The remaining cases are similar.
\end{proofof}
